A General Framework for Uncertainty Estimation in Deep Learning

Neural networks predictions are unreliable when the input sample is out of the training distribution or corrupted by noise. Being able to detect such failures automatically is fundamental to integrate deep learning algorithms into robotics. Current approaches for uncertainty estimation of neural networks require changes to the network and optimization process, typically ignore prior knowledge about the data, and tend to make over-simplifying assumptions which underestimate uncertainty. To address these limitations, we propose a novel framework for uncertainty estimation. Based on Bayesian belief networks and Monte-Carlo sampling, our framework not only fully models the different sources of prediction uncertainty, but also incorporates prior data information, e.g. sensor noise. We show theoretically that this gives us the ability to capture uncertainty better than existing methods. In addition, our framework has several desirable properties: (i) it is agnostic to the network architecture and task; (ii) it does not require changes in the optimization process; (iii) it can be applied to already trained architectures. We thoroughly validate the proposed framework through extensive experiments on both computer vision and control tasks, where we outperform previous methods by up to 23% in accuracy.

==> images/tick/test.tex <==
% This file was created by matplotlib2tikz v0.7.5.
\begin{tikzpicture}

\begin{axis}[
log basis y={10},
ytick={0.02,0.03,0.04,0.05,0.06,0.07,0.08,0.09,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,2,3,4,5,6,7,8,9,20,30,40,50,60,70,80,90,200,300,400,500,600,700,800,900},
yticklabels={\(\displaystyle {2\times10^{-2}}\),\(\displaystyle {3\times10^{-2}}\),\(\displaystyle {4\times10^{-2}}\),,\(\displaystyle {6\times10^{-2}}\),,,,\(\displaystyle {2\times10^{-1}}\),\(\displaystyle {3\times10^{-1}}\),\(\displaystyle {4\times10^{-1}}\),,\(\displaystyle {6\times10^{-1}}\),,,,\(\displaystyle {2\times10^{0}}\),\(\displaystyle {3\times10^{0}}\),\(\displaystyle {4\times10^{0}}\),,\(\displaystyle {6\times10^{0}}\),,,,\(\displaystyle {2\times10^{1}}\),\(\displaystyle {3\times10^{1}}\),\(\displaystyle {4\times10^{1}}\),,\(\displaystyle {6\times10^{1}}\),,,,\(\displaystyle {2\times10^{2}}\),\(\displaystyle {3\times10^{2}}\),\(\displaystyle {4\times10^{2}}\),,\(\displaystyle {6\times10^{2}}\),,,},
tick align=outside,
tick pos=left,
x grid style={white!69.01960784313725!black},
xlabel={T samples},
xmin=-0.15, xmax=47.15,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={log-likelihood},
ymin=0.120829448704748, ymax=1.07759092154894,
ymode=log,
ytick style={color=black},
ytick={0.01,0.1,1,10,100},
yticklabels={\(\displaystyle {10^{-2}}\),\(\displaystyle {10^{-1}}\),\(\displaystyle {10^{0}}\),\(\displaystyle {10^{1}}\),\(\displaystyle {10^{2}}\)}
]
\addplot [semithick, green!50.0!black]
table {%
2 -61.837898
3 -5.048196
4 -1.915031
5 -1.036674
6 0.133465
7 0.327378
8 0.639605
9 0.645324
10 0.70801
11 0.828999
12 0.826531
13 0.779083
14 0.857916
15 0.901801
16 0.859145
17 0.891001
18 0.948807
19 0.927595
20 0.912076
25 0.932818
30 0.95106
35 0.967653
40 0.975572
45 0.970197
};
\end{axis}

\begin{axis}[
axis y line=right,
tick align=outside,
x grid style={white!69.01960784313725!black},
xmajorgrids,
xmin=-0.15, xmax=47.15,
xtick pos=left,
xtick style={color=black},
y grid style={white!69.01960784313725!black},
ylabel={time},
ymajorgrids,
ymin=-0.000308500000000001, ymax=0.2549465,
ytick pos=right,
ytick style={color=black},
ytick={-0.05,0,0.05,0.1,0.15,0.2,0.25,0.3},
yticklabels={−0.05,0.00,0.05,0.10,0.15,0.20,0.25,0.30}
]
\addplot [semithick, blue]
table {%
2 0.011294
3 0.016515
4 0.022031
5 0.02755
6 0.033059
7 0.038531
8 0.043864
9 0.048856
10 0.054251
11 0.059707
12 0.06512
13 0.070602
14 0.076027
15 0.081365
16 0.088663
17 0.095007
18 0.100439
19 0.106042
20 0.111587
25 0.139322
30 0.16703
35 0.192478
40 0.219755
45 0.243344
};
\end{axis}

\end{tikzpicture}
